Proximal gradient methods with inexact oracle of degree q for composite optimization

We introduce the concept of inexact first-order oracle of degree q for a possibly nonconvex and nonsmooth function, which naturally appears in the context of approximate gradient, weak level of smoothness and other situations. Our definition is less conservative than those found in the existing literature, and it can be viewed as an interpolation between fully exact and the existing inexact first-order oracle definitions. We analyze the convergence behavior of a (fast) inexact proximal gradient method using such an oracle for solving (non)convex composite minimization problems. We derive complexity estimates and study the dependence between the accuracy of the oracle and the desired accuracy of the gradient or of the objective function. Our results show that better rates can be obtained both theoretically and in numerical simulations when q is large.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{AgKam:17}
A. Agafonov, D. Kamzolov, P. Dvurechensky, A. Gasnikov, and M. Takac,  \emph{Inexact Tensor Methods and Their Application to Stochastic Convex Optimization}, arXiv: 2012.15636v3, 2017.



\bibitem{Bec:17}
A. Beck, \emph{First-order methods in optimization}, vol. 25, SIAM, 2073.


\bibitem{BoGuRa:16}
L.Bogolubsky, G. Gusev, A. Raigorodskii, A. Tikhonov, M. Zhukovskii, P. Dvurechensky, A. Gasnikov, Y. Nesterov, \emph{ Learning supervised PageRank with gradient-based and gradient-free optimization methods}, 30th Conference on Neural Information Processing Systems, 2016, Barcelona, Spain.


\bibitem{Bot:10}
 Bottou L., \emph{Large-scale machine learning with stochastic gradient descent}, Proceedings of COMPSTAT, 177--186, 2010.



\bibitem{CoDiOr:18}
M. B. Cohen, J. Diakonikolas and L. Orecchia, \emph{On Acceleration with Noise-Corrupted Gradients}, International Conference on Machine Learning, Stockholm, Sweden, PMLR 80, 2018.  


\bibitem{Asp:08}
A. d’Aspremont,  \emph{ Smooth optimization with approximate gradient}, SIAM J. on Optimization, 19(3):1171--1183, 2008.



\bibitem{DeGlNe:13}
O. Devolder, F. Glineur, Y. Nesterov, \emph{First-order methods of smooth convex optimization
with inexact oracle}, Math. Program., Ser. A (2014) 146:37--75, 2013.



\bibitem{DvGa:16}
P. Dvurechensky and A. Gasnikov, \emph{Stochastic intermediate gradient method for convex problems with stochastic inexact oracle}, Journal of Optimization Theory and Applications, 171(1):121--145, 2016.



\bibitem{Dvur:17}
P. Dvurechensky,	\emph{ A gradient method with inexact oracle for composite nonconvex optimization}, Computer Research and Modeling, 14 NO. 2: 321--34, 2022.


\bibitem{KanLe:22}
C.Kanzow and T.Lechner,  \emph{Efficient regularized quasi-Newton methods for large-scale nonconvex composite optimization problems}, 2022.


\bibitem{Nes:04}
Yu.  Nesterov, \emph{Introductory lectures on convex optimization: A basic course},  Springer, 2004.


\bibitem{Nes:13}
Yu.  Nesterov, \emph{Gradient methods for minimizing composite functions}
Mathematical programming 140.1, 125--161, 2013.


\bibitem{Pol:63}
B.T. Polyak, \emph{Gradient methods for the minimisation of functionals}, USSR Computational Mathematics and Mathematical Physics 3.4 (1963): 864-878.

\bibitem{Sch:05}
M. Schmidt, \emph{Least squares optimization with $L_1$-Norm regularization}, CS542B Project Report, 2005.


\bibitem{StDv:19}
F. S. Stonyakin, D. Dvinskikh, P. Dvurechensky, A. Kroshnin, O. Kuznetsova, A. Agafonov, A. Gasnikov, A. Tyurin, C. A. Uribe, D. Pasechnyuk and S. Artamonov,  \emph{Gradient methods for problems with inexact model of the objective}, Mathematical Optimization Theory and Operations Research, 2019, Volume 11548.


\bibitem{Tib:96}
R. Tibshirani, \emph{Regression Shrinkage and Selection via the Lasso}, Journal of the Royal Statistical Society. Series B (Methodological), Vol. 58, No. 1, 267--288, 1996.

\bibitem{WaLI:14}
P.W. Wang and C-J. Lin, \emph{Iteration complexity of feasible descent methods for convex optimization}, J. Mach. Learn. Res. 15(4), 1523--1548, 2014.

\end{thebibliography}


